Faithful Explanations of Black-box NLP Models Using LLM-generated Counterfactuals

Causal explanations of the predictions of NLP systems are essential to ensure safety and establish trust. Yet, existing methods often fall short of explaining model predictions effectively or efficiently and are often model-specific. In this paper, we address model-agnostic explanations, proposing two approaches for counterfactual (CF) approximation. The first approach is CF generation, where a large language model (LLM) is prompted to change a specific text concept while keeping confounding concepts unchanged. While this approach is demonstrated to be very effective, applying LLM at inference-time is costly. We hence present a second approach based on matching, and propose a method that is guided by an LLM at training-time and learns a dedicated embedding space. This space is faithful to a given causal graph and effectively serves to identify matches that approximate CFs. After showing theoretically that approximating CFs is required in order to construct faithful explanations, we benchmark our approaches and explain several models, including LLMs with billions of parameters. Our empirical results demonstrate the excellent performance of CF generation models as model-agnostic explainers. Moreover, our matching approach, which requires far less test-time resources, also provides effective explanations, surpassing many baselines. We also find that Top-K techniques universally improve every tested method. Finally, we showcase the potential of LLMs in constructing new benchmarks for model explanation and subsequently validate our conclusions. Our work illuminates new pathways for efficient and accurate approaches to interpreting NLP systems.

==> 3.method.tex <==
\section{Method}
\label{sec:method}

\subsection{Model explanation with counterfactuals}
\label{sub:counterfactuals}
% \amit{The order of material in this subsection  can be improved. How about a) we first define CACE and ICACE and say that this is the basis of causal explanation as per past work; b) say that CF generation (and matching) is one way to achieve these metrics, because we need to estimate t' ; c) say that before we present the methods, let us first show why causal explanation based on CFs is ideal. }
This study focuses on model explanation with \textit{counterfactuals (CFs)}, which enables causal estimation in a model-agnostic manner (because CFs do not depend on the explained model). While we are aware of the causal graph that encodes our causal assumptions, for a given problem we cannot access the complete data-generating process (DGP) nor the variable values of an example, and therefore, we cannot produce gold CFs. Given this, we propose two approaches for approximating them.

The first approach we introduce is \textit{Counterfactual generation}, in which a generative model (an LLM) is prompted to change an attribute conveyed in the text while holding confounding attributes fixed. Nevertheless, utilizing an LLM at inference time is frequently impractical because of its prolonged latency, high financial costs, or privacy concerns that prevent data from being sent to external servers (see the discussion in \citet{kd_nlg} and our latency measurements in \S\ref{app_sub:efficiency}). 

Considering these challenges, we introduce an efficient alternative, the \textit{matching} technique. This approach aims to find CF approximations within a pre-defined candidate set. To further enhance the matching process, we propose a novel method that leverages CFs generated by an LLM during training time \textit{for learning causal representations} that are faithful to the causal graph. 

\input{tables/sets_example}
\vspace{-0.25cm}

To provide an accurate causal explanation, we should estimate the \textit{Average Treatment Effect (ATE)} \citep{causality} or the \textit{Individual Treatment Effect (ITE)}  \citep{shpitser2006identification,ite}. Specifically, the treatment is a high-level concept describing the text (such as \textit{ambiance} in a restaurant review), and the outcome variable is a prediction of a text classifier (e.g., see the causal graph in Figure~\ref{fig:causal_graph}). When discussing model explanation in the sense of the causal effect of a concept on the model prediction, the common versions of the ATE and the ITE are the \textit{Causal Concept Effect (CaCE)} \citep{cace} and the \textit{Individual Causal Concept Effect (ICaCE)} \citep{cebab}.
 
Given a DGP $\gG$, an intervention on a treatment variable $T: t \rightarrow t'$ (for simplicity we sometimes write $T \leftarrow t'$), a model $f$, and an input example $\vx_t$, the CaCE and ICaCE are defined to be:
\begin{align}
\label{eq:formal_cace}
    \texttt{CaCE}_f(T, t, t') &= \E_{\vx' \sim \gG}\left[f(\vx')|do(T=t')\right] - \E_{\vx' \sim \gG}\left[f(\vx')|do(T=t)\right] 
    \\
    \texttt{ICaCE}_f(\vx_t, T, t') &= \E_{\vx' \sim \gG}\left[f(\vx')|\vx_t, do(T=t')\right] - f(\vx_t) \nonumber
\end{align}
If $\widetilde{\vx}_{t'}$ is an approximated CF of the text $\vx_{t}$ resulted from the intervention $T: t \rightarrow t'$ (can be either a model-generated CF or a match), then the causal effect estimators are:
\begin{align}
\label{eq:icace}
    \icace(\vx_t, T, t, t') &:= \icace(\vx_t, \widetilde{\vx}_{t'}) = f(\widetilde{\vx}_{t'}) - f(\vx_t) \\
    \cace(T, t, t') &= \frac{1}{|\sD|}\left( 
    \sum_{\vx_t}{\icace(\vx_t, \widetilde{\vx}_{t'})} +
    \sum_{\vx_{t'}}{\icace(\widetilde{\vx}_{t}, \vx_{t'})} +
    \sum_{\vx}{\icace(\widetilde{\vx}_{t}, \widetilde{\vx}_{t'})}
    \right) \nonumber
\end{align}
\textbf{Counterfactuals as an ideal model explanation.}
Faithfulness, the ability of an explanation method to accurately describe a model's underlying reasoning, lacks a consistent definition in the literature \citep{faithfulness3, jacovi2020towards, faithfulness1, faithful_survey}. In this paper, we introduce a simple, intuitive, and essential criterion: \textit{Order-faithfulness}. This implies that if the explanation method ranks the impact of one concept (or intervention) higher than another, the true causal effect of the first concept should genuinely exceed that of the second. Order-faithfulness is crucial in scenarios like model selection and deployment. For instance, to determine the fairness of a hiring model, it is essential to know whether it incorrectly prioritizes non-relevant concepts (e.g., gender) over genuine concepts (such as experience). We next formally define this necessary property. 

In Appendix \S\ref{sec:theorem} we provide detailed formal definitions of both approximated CFs and non-causal explanation methods. Furthermore, we prove (under reasonable assumptions) the following theorem, which elucidates why approximated CF methods are order-faithful, unlike non-causal ones.

\begin{definition*}[Order-Faithfulness]
Given an i.i.d. dataset $\sD$ sampled from a DGP $\gG$, an explained model $f$ and two interventions $C_1: c_1 \rightarrow c'_1, C_2: c_2 \rightarrow c'_2$, an explanation method $S$ is \textbf{order-faithful} if: 
\begin{align}
    \E_{\sD \sim \gG}[S(f, C_1, c_1, c'_1)] > \E_{\sD \sim \gG}[S(f, C_2, c_2, c'_2)] \Longleftrightarrow \texttt{CaCE}_{f}(C_1, c_1, c'_1) > \texttt{CaCE}_{f}(C_2, c_2, c'_2) 
% \label{eq:strong}
% S(f, \vx, C_1 \leftarrow c'_1) > S(f, \vx, C_2 \leftarrow c'_2) \Longleftrightarrow \texttt{ICaCE}_{f}(\vx, C_1, c'_1) > \texttt{ICaCE}_{f}(\vx, C_2, c'_2) 
\end{align}
\end{definition*}
\begin{theorem*}
For an explained model $f$, (1)  The approximated CF explanation method $S_{CF}$ is order-faithful for every DGP $\gG$ and two interventions; (2) For every DGP $\gG$, there exist a DGP $\gG'$ resulting from a small modification of $\gG$, a model $f'$, and two interventions $C_1: c_1 \rightarrow c'_1, C_2: c_2 \rightarrow c'_2$ such that the non-causal explanation method $S_{NC}$ is not order-faithful.
\end{theorem*}
% \textit{Proof sketch}: We first show that approximated CF methods are always faithful. Then, we construct $\gG'$ by introducing a new unobserved confounder variable that reverses the causal effect. 
% In addition, we ensure that the non-causal method produces the same explanations as it produces for $\gG$, and therefore, it cannot be order-faithful in $\gG$ and $\gG'$ at the same time. 
In Appendix~\ref{sec:theorem} we define the explanation methods $S_{CF}$ and $S_{NC}$ and describe what is ``a small modification''. The theorem underscores the importance of developing causal-inspired explanation methods and suggests why our CF-based approaches are more effective than other baselines. 
% \amit{it will be good to some more justification/interpretation of the theoretical result. For example, we may first give intuitive description of the faithfulness defn. We can say it holds for comparing the importance of two concepts, as attribution methods like LIME do, and it also  holds for comparing the importance of changes in same concept. For the theorem, it will be helpful to add a proof sketch just below it. E.g. Proof Sketch. We first show that approx CF explanation is always faithful. Then we show that non-causal explanation may rely on confounded replationships since it only depends on observed data, and hence construct a dataset where non-causal explanation will be not faithful. }

\subsection{Causal representation learning for matching}
\label{sub:causal_representation}

% A matching method should account for the following steps: 

% \begin{enumerate}
%     \item Representing examples as a numeric vector - Considering the causal graph and deciding which variables should be included and how to map discrete or categorical variables (such as text) into a continuous vector.
%     \item Ranking the candidates according to their ``closeness'' to the query example - Defining what is ``closeness'' and which measure should be used to compute it.
%     \item Aggregating the ranked list into an estimator - This includes choices such as the number of matches, weighting, and deciding on matching with or without replacement.
% \end{enumerate}

% We focus on the first step and propose a method for learning causal representations that improve the matching. We chose to highlight this stage because, unlike the other stages, it is distinctive to NLP due to the discrete nature of texts and remains relatively uncharted in this field. For the second and third steps, 

Although counterfactual generation is a valuable model explanation approach, employing LLMs during inference can be infeasible. Conversely, there is an opportunity to harness model-generated CFs to train an efficient method that seeks approximations within a pre-defined set of candidate texts, mitigating the need for direct generation. This approach is known as \textit{matching} \citep{matching} and endeavors to match each treatment unit with its most similar control unit. To allow effective matching, we introduce a novel method that learns to encode texts in a space faithful to the causal graph, i.e., each treatment unit resonates closely with its 
CF counterparts and remains distinct from confounding texts. Formally, a matched example of $\vx_t$ is defined to be:
\begin{align}
\label{eq:match}
    m_1(\vx_t) = \argmax_{\vx_{t'} \in \sD(T=t')}{s\left(\phi(\vx_t), \phi(\vx_{t'})\right)}
\end{align}
The \textit{candidate set} is denoted by $\sD(T=t')$ and is also known as the control group, contains only texts whose treatment variable equals $t'$, and is known in advance (i.e., both the treatment and control groups are pre-defined and there is no need to infer which text belong to which group). $\phi(\cdot)$ is a feature extractor function (the language representation model we aim to learn) that maps discrete text to the hypersphere space where matching is conducted by ranking candidates according to their cosine similarity (see Eq.~\ref{eq:cosine}) with the query example: $s(\phi(\vx_t), \phi(\texttt{candidate}))$. Notice that Eq~\ref{eq:match} defines \textit{1:1 matching}, but we also experiment with \textit{Top-$K$ matching}: $\frac{1}{K}\sum_{i=1}^{K}\icace(\vx_t, m_i(\vx_t))$. 

Our causal representation method is based on an Encoder-only language model (e.g., RoBERTa \citep{roberta} or a SentenceTransformer \citep{starnsformer} in our case) fine-tuned to minimize an objective consisting of six contrastive loss components. The goal of the objective is to enhance the similarity with approximate counterfactuals and matches while reducing similarity with misspecified counterfactuals and matches. 

Given a causal graph, an intervention on a treatment variable $T:t \rightarrow t'$ and an example $\vx_t$, we define the four following sets (see toy examples in Table~\ref{tab:set_exmamples}): 
\begin{enumerate}[nosep]
    \item $\XCF$ - This set contains \textit{Counterfactuals}, obtained by modifying $\vx_t$ through the intervention on $T$, while the other variables are held unchanged. We utilize an LLM (ChatGPT) to simulate several CFs (up to ten). 
    
    \item $\XM$ - This set contains \textit{Matched samples}. These instances share identical values for the adjustment variables (that satisfy the back-door criterion, see Appendix \S\ref{app:formulations}). Our study employs a smaller model to predict their values and construct a set of valid matches.
    
    \item $\XMiCF$ - This set contains \textit{Misspecified Counterfactuals}. These examples are derived from editing $\vx_t$ through interventions on variables other than the treatment variable. The term \textit{misspecification} is well-known in the causal literature and indicates a wrong assumption of the DGP \citep{miss}. In our case, a wrong intervention.
    
    \item $\XMiM$ - This set contains \textit{Misspecified Matched samples}. This is the complementary set to $\XM$, containing all those instances that do not qualify as valid matches due to differing values of the adjustment variables. 
\end{enumerate}
We next formulate the \textit{contrastive loss} \citet{contrastive}, which aims to attract some input $\vx$ to the ``positive set'' $\sX_+$, and separate it from the ``negative set'' $\sX_-$. $\tau$ is a temperature hyperparameter.
% some input example $\vx$, a set of examples $\sX_+$ that $\vx$ should be attracted to, and a set of examples $\sX_-$ that $\vx$ should be separated from:
\begin{align}
\label{eq:contrastive}
    \mathcal{L}(\vx, \sX_+, \sX_-) = -\log \left[ \frac{\sum_{\vx_+}{\exp(s(\phi(\vx), \phi(\vx_+)) / \tau)}}{\sum_{\vx_+}{\exp(s(\phi(\vx), \phi(\vx_+)) / \tau)} + \sum_{\vx_-}{\exp(s(\phi(\vx), \phi(\vx_-)) / \tau})} \right]
\end{align}
The final loss consists of six contrastive loss components:
% \begin{align}
%     \mathcal{L}(\vx_t) = & \mathcal{L}(\vx_t, \XCF, \XMiM) + \mathcal{L}(\vx_t, \XCF, \XMiCF) + \mathcal{L}(\vx_t, \XCF, \XM)  \label{eq:loss} \\ 
%  + & \mathcal{L}(\vx_t, \XM, \XMiM) + \mathcal{L}(\vx_t, \XM, \XMiCF) 
%     + \mathcal{L}(\vx_t, \XMiCF, \XMiM) \notag
% \end{align}
\begin{align}
    \mathcal{L}(\vx_t) = & \mathcal{L}(\vx_t, \XCF, \XMiM) + \mathcal{L}(\vx_t, \XCF, \XMiCF) + \mathcal{L}(\vx_t, \XCF, \XM)  \notag \\ 
 + & \mathcal{L}(\vx_t, \XM, \XMiM) + \mathcal{L}(\vx_t, \XM, \XMiCF) \label{eq:loss} \\
    + & \mathcal{L}(\vx_t, \XMiCF, \XMiM) \notag 
\end{align}
% We hypothesize (and verify in our ablation study at \S\ref{sub:ablation}) that a similarity function that utilizes representations drawn from a model $\phi(\cdot)$ which minimizes the objective Eq.\ref{eq:loss}, would be an effective matching function. Accordingly, our method prefers texts that most closely resemble CF approximations within a pre-defined candidate set. In the lack of CFs, the method defaults to matching texts with the same adjusting variable values. When choosing between misspecified CFs or misspecified matches, the methods favor the latter, given their potential shared traits with the CF, such as syntax or style linked to exogenous variables.
% Formally, given a query example $\vx_t$ and four matching candidates $\xCF \in \XCF, \xM \in \XM, \xMiCF \in \XMiCF$, the candidates' ranking, which is based on their similarity with $\vx_t$, should be $\xMiM \preceq  \xMiCF \preceq \xM \preceq \xCF$. This desirable order is not arbitrary and is a direct product of the six components of the objective (Eq.\ref{eq:loss}). Absent any of these components, the representation risks favoring inaccurate matches, as we highlight in the ablation study. Crucially, these six components also ensure the robustness of our causal representation model to variations of the candidate set, for example, in case it contains golden CFs or misspecified CFs. Robustness is vital, as we cannot make assumptions about the candidate set.
\textbf{We hypothesize (and verify) that omitting components from the objective risks favoring inaccurate matches, as we highlight in the ablation study at \S\ref{sub:ablation}.} Accordingly, the objective prioritizes text matches that closely resemble CF approximations within a candidate set, defaulting to adjusting variable values in their absence. When choosing between misspecified CFs or misspecified matches, the methods favor the latter, given their potential shared traits with the CF, such as syntax or style linked to exogenous variables. Formally, given a query example $\vx_t$ and four matching candidates $\xCF \in \XCF, \xM \in \XM, \xMiCF \in \XMiCF$, the candidates' ranking, which is based on their similarity with $\vx_t$, should be $\xMiM \preceq  \xMiCF \preceq \xM \preceq \xCF$. This desirable order is not arbitrary and is a direct product of the six components, ensuring robustness to variations of the candidate set.

\textbf{Training procedure.} We start with a small set of textual examples (the train set) labeled with the adjusting variables (e.g., review concepts such as food and service). Initially, we employ a small Encoder-only model (RoBERTa) and train a concept predictor for each variable. The predictor models are then harnessed to construct the four sets: By predicting the concept values of each training example, we divide them (according to their concept values) and construct the $\XM$ and $\XMiM$ sets. 

For constructing $\XCF$ and $\XMiCF$, we use a few-shot LLM (ChatGPT) to generate approximate CFs and misspecified CFs (see prompts at \S\ref{app_sub:prompts}). We filter out misspecified CFs from $\XCF$ if the concept predictors indicate an adjusted variable was also changed during the treatment intervention. Additionally, we use simple rules to filter unsuccessful generations (e.g., empty strings, ``As an AI LM...''). 

To train our language representation model (aimed to explain a specific concept), we proceed as follows: For every training example $\vx_t$, we randomly sample four examples: $\xCF \in \XCF, \xM \in \XM, \xMiCF \in \XMiCF$. The training goal is to minimize the objective of Eq.~\ref{eq:loss}. We repeat this process for several epochs (15) and select the checkpoint that achieves the lowest loss on the dev. set.

==> 4.experimental.tex <==
% \input{figures/causal_graph_tex}

\section{Experimental setup}
\label{sec:experimental}

\subsection{Model explanation pipeline}
\label{sub:explanation_pipeline}

\textbf{Causal Estimation-Based Benchmark (CEBaB).} CEBaB \citep{cebab} comprises high-quality, labeled CFs designed to benchmark model explanation methods. This benchmark originated from thousands of original restaurant reviews obtained from OpenTable. For every original review, human annotators were tasked to edit the review and write an approximate CF that reflects a specific intervention, e.g., ``change the service concept from positive to negative''. Each entry (original reviews and approximate CFs) in CEBaB received a 5-star sentiment rating, labeled by five annotators. Furthermore, every text was annotated at a conceptual level, as positive, negative or neutral w.r.t. four central mediating concepts: Food, Service, Ambiance, and Noise (see Figure~\ref{fig:causal_graph}). CEBaB contains two train sets, exclusive ($N=1463$) and inclusive (which we do not use), development ($N=1672$), and test ($N=1688$) sets. We randomly split the exclusive set into two equal sets: the train set (for training the causal representation model and the concept predictors) and a matching candidates set.

\textbf{Evaluation measures.} CEBaB allows estimating the CaCE and ICaCE by plugging the human-written CF, $\widetilde{\vx}^h_{t'}$, into the $\icace$ estimator: $\icace(\vx_t, \widetilde{\vx}^h_{t'})$
This is the difference between the outputs of the model $f$ (a five-dimension vector in CEBaB). The CEBaB ICaCE allows evaluating an explanation method $m$ by computing errors w.r.t. an intervention:
\begin{align}
\label{eq:error}
   \err(f, m, T, t, t') = \frac{1}{|\sD(T \leftarrow t')|}\sum_{(\vx_t,\widetilde{\vx}^h_{t'}) \in \sD} {\texttt{Dist} \left( \icace(\vx_t, \widetilde{\vx}^h_{t'}), \icace(\vx_t, \widetilde{\vx}^m_{t'}) \right)}
\end{align}
Where $\texttt{Dist}$ can be, for example, the $L2$ distance, the cosine distance ($1-\cos$), or the norm difference (see \citet{cebab} for more details). The $\err$ scores we present in this study are the mean over 24 interventions: four concepts with three values (six interventions for each concept). 

\textbf{Evaluation pipeline.} For the generative approach, we generate a CF $\widetilde{\vx}^m_{t'}$ using an LLM and calculate $\icace(\vx_t, \widetilde{\vx}^m_{t'})$. For matching, given an intervention $T \leftarrow t'$ and a set of candidates that share the new treatment value: $\sD(T=t') = \left\{\vx|\vx \in \sD, T(\vx)=t' \right\}$, we utilize a matching model (e.g., our causal representation model) to represent each candidate with a high-dimensional continuous vector. To this end, we extract the last layer hidden states of the candidate's tokens and compute their mean vector. Finally, given a query example $\vx_t$, we extract its representation, rank the candidates according to their cosine similarity, select a match, and calculate the $\icace(\vx_t, m_1(\vx_t))$.

\subsection{Models and baselines}
\label{sub:baselines}

In \Cref{app:implementations} we provide additional implementation details, including hyparameters and prompts.

\textbf{Generative approach.} We employ three different CF generation techniques: \textit{Zero-shot Generative}, \textit{Few-shot Generative} (with three demonstrations) and \emph{Fine-tune Generative}. The first two are based on the Decoder-only ChatGPT \citep{chatgpt}, while the third is based on an Encoder-decoder T5-base model \citep{t5} trained using a parallel dataset, comprised of original reviews and their human-written CFs (the inclusive train set of CEBaB). The zero-shot and few-shot prompts are described in Appendix \S\ref{app_sub:prompts}. 

\textbf{Matching baselines.} We benchmark against six matching methods: (1) \textit{Random Match}, which randomly selects an example from the candidate set; 
(2) \textit{Propensity} \citep{propensity}, which first estimates the propensity score $P(T=t'|x)$ using a concept predictor, and then conducts matching based on this score;
(3) \textit{Approx}, which randomly selects an example from $\XM$. Notice that $\XM$ can be an empty set, thus, unlike the other baselines, matching may not be performed;
(4) \textit{PT RoBERTa}, which utilizes a pre-trained LM to represent texts and finds matches using their cos similarity;
(5) \textit{PT S-Transformer}, same as PT RoBERTa, expect the backbone model is a SentenceTransformer model \citep{starnsformer} trained to maximize semantic textual similarity; 
and (6) \textit{FT S-Transformer}, a SentenceTransformer fine-tuned to predict the five-star sentiment; \\
Notice that \citet{cebab} found that Approx outperforms all seven tested (non-matching) baselines (see Figure~\ref{fig:cebab_barplot}). Therefore we do not include them in this study.

\textbf{Interpreted models.} We interpret five different models of varying sizes. The first three are Encoder-only models fine-tuned using only the original reviews from the train set of CEBaB to predict the five-star sentiment. These models include DistilBERT \citep{distilbert}, BERT \citep{bert}, and RoBERTa \citep{roberta}. The other two are the zero-shot chat versions of the Decoder-only Llama-2 model \citep{llama2} with 7 and 13 billion parameters. We extract the five-star sentiment distribution of the Llama models using the prompt described in Figure~\ref{fig:rating}. 

% \subsection{Implementation Details}
% \label{sub:implementations}

% We use $\tau=0.1$, train the causal representation models for 12 epochs, and select the model checkpoint which minimizes the objective of Eq.~\ref{eq:loss} (or its modified version for the ablation models). Notice that when using the $\err$ as the selection criterion, one might be able to select a more robust checkpoint. However, this violates the model-agnostic property, as calculating the $\err$ requires access to the explained model. The backbone SentenceTransformer of our model is MPNet (\texttt{all-mpnet-base-v2}) \citep{mpnet}.
% We use a learning rate of 5e-6 for training the causal representation models. We use a learning rate of 1e-5 and a batch size of 16 for the fine-tuned baselines, explained models and concept predictors. The concept predictor models are used for filtering misspecified CFs (for constructing the $\XCF$ and $\XMiCF$ sets) and for the Approx and Propensity score baselines. We fine-tune a RoBERTa model using the annotated train set for each of the four concepts.

==> 6.new_setup.tex <==
\section{New Setup: Explaining Stance Detection Models}
\label{sec:new_setup}

While we aim to validate our earlier conclusions across multiple benchmarks, CEBaB remains the sole high-quality benchmark for NLP explainers. On the other hand, we show that LLMs generate CFs that resemble human-written CFs. Consequently, we harness LLM capabilities to emulate CEBaB and propose a new benchmark for model explanation, eliminating the high cost of manually annotating such benchmarks. We decided to focus on Stance Detection, which is an important and well-studied NLP task that determines the position (support, oppose, neutral) expressed by the speaker towards a particular topic (e.g., abortions, climate change) \citep{stance_detection_survey, stance_detection_miss, stance_detection1}. This task is intriguing because understanding public opinions and beliefs can guide decision-making, policy formulation, and marketing strategies. Estimating the causal effect of high-level concepts like gender or age may shed light on the societal biases and perceptions that drive social trends.

We rely on the stance detection dataset from the SemEval 2016 shared task \citep{semeval16}. This dataset contains tweets about five subjects: Abortion, atheism, climate change, feminism, and Hillary Clinton. Humans annotated the stance of the tweets with three possible labels: support, oppose, and neutral. 
For simplicity of the new setup, we embrace the same causal graph of CEBaB (see Figure~\ref{fig:causal_graph}), but replace the four review concepts with new relevant concepts: (1) Tweet's subject (specified above); (2) Speaker's age - teenage, elder or unknown; (3) Speaker's gender - female, male or unknown; and (4) Speaker's Job - farmer, professor or unknown. The four concepts have an exogenous variable $U$ as their parent and are the direct cause of the text $X$ and the label (stance) $Y$, which is naturally affected by the four concepts. The explanation methods should estimate the effect of 9 interventions: changing the value of the three speaker's traits (age, gender, job) to three values. 

\paragraph{Constructing the new setup.} We follow three steps for constructing the new benchmark. In the first stage, we randomly split the data into four sets: train ($N=1000$), matching ($N=2000$), dev ($N=200$), and test ($N=500$). Each subject is precisely one-fifth of each split. For each set and subject, we keep 30\% of the original tweet and assign an `unknown' value to the speaker's concepts. For the remaining 70\%, we randomly (but not uniformly since we want to introduce correlations between the concepts and the label) sample two of the three speaker's concepts and assign new values (e.g., male, unknown age, professor).
In the second stage, we utilize GPT-4 to generate new tweets according to the new value assignment of 70\% of the tweets. The prompts we used are described in Figure~\ref{}. 
In the third and final stage, we utilize GPT-4 to generate the ground-truth CFs for the test set, which enables calculating the $\err$ for evaluating explanation methods. Accordingly, for each test example, we prompt GPT-4 and generate a single CF for each of the six possible interventions (3 speaker's concepts with two possible values that are different from the assignment). 

\paragraph{Experimental details.} We explain two stance detection fine-tuned RoBERTa models. The first is when on labels of the original tweets and the second is when fine-tuning on the new labels extracted by GPT-4. For the CF generation approach, we employ ChatGPT (and not GPT-4 which generates the ground-truth CFs of the test set) and only with zero-shot prompts. We benchmark our causal representation model with the same matching baselines from \S\ref{sub:baselines} with the same hyperparameters and training procedure described in \S\ref{sub:implementations}.

\input{tables/new_setup_results}

\paragraph{Results.} We report the results on Table~\ref{tab:new_results}. As can be seen, we reproduce our main findings from the previous section on the new benchmark, confirming the robustness of our conclusions. Specifically, the generative approach outperforms the matching methods (although consider that in this setup, the ground-truth CFs are also model-generated). In addition, our causal representation model surpasses the other matching baseline and outperforms the generative model when the candidate set contains ground-truth CFs. Finally, the Top-$K$ technique universally improves all the explainers. 



==> c.theorem.tex <==



Faithfulness is crucial in scenarios like model selection and deployment, especially for automatic decision-making systems.

However, there is no consistent formal definition of faithfulness in the literature \citep{jacovi2020towards}. 
\alex{We may emphasize here or later that usually, those definitions require an explanation of the model altogether, which may be impossible for such complex models as LLMs}.
No one is talking about specific interventions or concept importance. Usually, they assume that the explanation is robust and explains the whole reasoning process. For example, requiring that examples with the same explanations have the exact prediction or that the model may be reduced to some rule set.

For example, \citet{faithfulness1} concentrate on the alignment of explanations with predictions and separate faithfulness to consistency and sufficiency, assuming that the explanation can be used as a proxy for the prediction. \citep{faithfulness_health}) call faithfulness "fidelity" and require completeness and soundness, reasoning that the explanation describes the entire dynamic of the task model. \citep{jacovi2020towards} attempt to encapsulate various definitions of faithfulness by formulating assumptions underlying methods used for (dis)proving the faithfulness of specific methods. 

In this work, instead of focusing on the ability of a method to provide a complete and accurate explanation of a complex model, we focus on the importance of concepts for such a model. Using that importance may be formulated as a single number we \textbf{formally} define the faithfulness of an explanation method to a specific concept, the property we call \textit{order-faithfulness}. Essentially, an explanation method is order-faithful if it ranks the impact of one concept (or intervention) higher than another if and only if the true causal effect of the first concept should exceed that of the second. For instance, to determine the fairness of a hiring model, it is essential to know whether it incorrectly prioritizes non-relevant concepts (e.g., gender) over genuine concepts (such as experience).


==> figures/causal_graph_tex.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/causal_graph.pdf}
    \caption{The causal graph describing the data generating process of CEBaB benchmark \citep{cebab}. $U$ and $V$ are exogenous variables representing the state of the world. For example, $V$ may account for style, syntax, and length. The four concepts $F$ (food), $S$ (service), $A$ (ambiance) and $N$ (noise) affect both the textual review $X$ and its five-star rating $Y$. The relationship between $X$ and $Y$ can be causal or anti-causal. 
    % The relationship between $X$ and $Y$ can be causal ($X \rightarrow Y$, e.g., the rating is provided by an annotator who reads the review) or anti-causal ($Y \rightarrow X$, e.g., the rating held by the reviewer shapes the content of the review they write). 
    $f$ is the model we wish to explain, which is trained to predict $Y$ from $X$. In this study, we are interested in estimating the causal effect of changing the value of an concept on the predictive model $f$ (e.g., changing the value of the red variable $S$ from positive to negative).}
    \label{fig:causal_graph}
\end{figure}

==> tables/new_setup_results.tex <==
\begin{table}[t!]
\captionof{table}{Examples from the new Stance Detection setup.
In the first stage of the dataset construction (top table), we split the original tweets into the train, dev, matching, and test sets. 
In the second stage (middle table), we keep 30\% of the original tweets, and for the remaining 70\%, we randomly assign values for the thee writer's concepts. In this example, we ask GPT-4 to edit the tweet ``to make it sound as if a teenage female wrote it''. In the third (bottom table), we generate CFs for the test set (and are used for benchmarking). In this example, we ask GPT-4 to change the Job concept to Farmer.}
\label{tab:new_setup_exmamples}
\begin{minipage}[b]{.54\textwidth}
\centering
\scriptsize
\begin{tabularx}{\textwidth}{ X }
\toprule
\textbf{S1: Original tweet.} $\hfill Subject: \texttt{Feminism}$ \\
$Age: \texttt{?} \hfill Gender: \texttt{?} \hfill Job: \texttt{?} \hfill Label: \texttt{Favor}$ \\
I need feminism because "what were you wearing" shouldn't be a question when I tell my stepmom I was cat called. \#SemST \\
\midrule
\textbf{S2: Modified tweet.} $\hfill Subject: \texttt{Feminism}$ \\
$Age \rightarrow \texttt{Teen} \hfill Gender \rightarrow \texttt{\female} \hfill Job: \texttt{?} \hfill Label: \texttt{Favor}$ \\
OMG, like, I totally need feminism cuz 'what were you wearing?' shouldn't even be a thing when I tell my stepmom some guy shouted stuff at me. \#JustSaying \\
\midrule
\textbf{S3: Counterfactual (for the test set).} $\hfill Subject: \texttt{Feminism}$ \\
$Age: \texttt{Teen} \hfill Gender: \texttt{\female} \hfill Job \rightarrow \texttt{Farmer} \hfill Label: \texttt{Favor}$ \\
Gosh, I reckon I'd holler for feminism, 'cause 'what were ya wearin?' ought not be a question when I tell ma about some fella yelled stuff at me while I was out in the fields. \#JustSaying \\
\bottomrule
\end{tabularx}
\end{minipage}
\hfill
\begin{minipage}[b]{.45\textwidth}
\centering
\large
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{l|ccc|ccc}
\toprule
 & \multicolumn{3}{c|}{\textbf{$K=1$}} & \multicolumn{3}{c}{\textbf{$K=10$}}
\\
 & \underline{\textit{L2}} & \underline{\textit{Cos}} & \underline{\textit{ND}} & \underline{\textit{L2}} & \underline{\textit{Cos}} & \underline{\textit{ND}}  
\\
\midrule
  Causal Model (+GT) &  \textbf{.13} &            \textbf{.09} &  \textbf{.06} & \textbf{.14} & \textbf{.10} & \textbf{.07}   \\
 \midrule
Zero-shot Generative &           .43 &            .35 &           .24 &          .47 &          .35 &          .25  \\
        \midrule
        Random Match &           .88 &            .64 &           .47 &          .96 &          .62 &          .49  \\
          Propensity &           .90 &            .68 &           .48 &          .99 &          .69 &          .56  \\
              Approx &           .74 &            .60 &           .41 &          .81 &          .58 &          .45  \\
          PT RoBERTa &           .75 &            .61 &           .39 &          .83 &          .59 &          .42   \\
    PT S-Transformer &           .75 &            .60 &           .40 &          .83 &          .60 &          .45  \\
    FT S-Transformer &           .72 &            .78 &           .46 &          .82 &          .79 &          .59  \\
        Causal Model &  \textbf{.66} &   \textbf{.55} &  \textbf{.36} & \textbf{.70} & \textbf{.55} & \textbf{.39} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{minipage}
\captionof{table}{Results for the new stance detection setup we introduce. We explain RoBERTa fine-tuned on the two topics: Climate Change and Feminism. The description of the rows is given in the caption of Table~\ref{tab:new_results}. \textbf{Numbers are the mean over 18 interventions, $\downarrow$ is better.}}
\label{tab:new_results}
\end{table}

